The role of binarity and stellar rotation in the split main sequence of NGC 2422

In addition to the extended main-sequence turnoffs widely found in young and intermediate-age (~ 600 Myr-2 Gyr-old) star clusters, some younger clusters even exhibit split main sequences (MSs). Different stellar rotation rates are proposed to account for the bifurcated MS pattern, with red and blue MSs (rMS and bMS) populated by fast and slowly rotating stars, respectively. Using photometry from Gaia Early Data Release 3, we report a Galactic open cluster with a bifurcated MS, NGC 2422 ( ~ 90 Myr). We exclude the possibilities that the bifurcated MS pattern is caused by photometric noise or differential reddening. We aim to examine if stellar rotation can account for the split MSs. We use spectra observed with the Canada-France-Hawaii Telescope and the Southern African Large Telescope, and directly measured v sin i, the projected rotational velocities, for stars populating the bMS and rMS. We find that their v sin i values are weakly correlated with their loci in the color-magnitude diagram because of contamination caused by a large fraction of rMS stars with low projected rotational velocities. Based on the spectral energy distribution fitting method, we suggest that these slowly rotating stars at the rMS may hide a binary companion, which breaks the expected v sin i-color correlation. Future time-domain studies focusing on whether these slowly rotating stars are radial velocity variables are crucial to test the roles of stellar rotation and binarity in generating the split MSs.

==> natbib.tex <==
%\documentclass[onecolumn]{aastex3}

\newcommand\aastex{AAS\TeX}%

\begin{document}

\begin{center}
Using {\tt\string natbib} with \aastex
\end{center}

\aastex\ uses Patrick Daly's {\tt\string natbib} package to manage
citations. The {\tt\string natbib} package re-implements LaTeX's
{\tt\string\cite} command, and offers greater flexibility for managing
citations in the author-year form. {\tt\string natbib} is required with the
\aastex\ package but fortunately {\tt\string natbib} is included in most
modern distributions. Authors are encouraged to read the {\tt\string
natbib} documentation for complete details on the package's capabilites.
All examples in this document are adapted from the {\tt\string natbib}
documentation.

Authors must use the LaTeX's {\tt\string thebibliography} environment to
use the {\tt\string natbib} extensions. Here is a bibliography with two
entries marked up in the {\tt\string natbib} style:

\begin{verbatim}
\begin{thebibliography}{}
\bibitem[James et al.(1991)]{jam91} James, H. ...
\bibitem[Jones et al.(1990)Jones, Baker, and Williams]{jon90} Jones, J. ...
\end{thebibliography}
\end{verbatim}

The square-bracketed argument contains the "author" portion of the citation
followed by the year in parentheses. The parentheses are important, so do
not leave them out. Note that in the second {\tt\string\bibitem}, the
square-bracketed argument includes two author lists, a short version before
the year and a long version after. Authors should use this form of the
markup if they wish to use the * forms of the {\tt\string\cite} commands.
(See the examples below.)

The text in the curly-brace argument of the {\tt\string\bibitem} is the
citation key and should be used as the argument in the corresponding cite
commands in the text. The two basic text citation commands are
{\tt\string\citet} and {\tt\string\citep}. ({\tt\string\citet} corresponds
to the plain LaTeX {\tt\string\cite} command.) Use the two optional
arguments to append text before or after the citationtext in the first set
of square brackets will appear before the cite, text in the second set will
appear after it. Use the asterisk (*) form of the cite commands to print
the long version of the author lists for references that have been marked
up in the manner of the "jon90" example.

Here are some {\tt\string\citet} and {\tt\string\citep} examples taken from
the {\tt\string natbib} package
documentation\footnote{\url{http://www.ctan.org/pkg/natbib}}.

\begin{tabular}{ll}
\textbf{Command} & \textbf{Output} \\
\verb|\citet{jon90}| & Jones et al. (1990) \\
\verb|\citet[chap.~2]{jon90}| & Jones et al. (1990, chap.~2) \\
\verb|\citep{jon90}| & (Jones et al., 1990) \\
\verb|\citep[chap.~2]{jon90}| & (Jones et al., 1990, chap.~2) \\
\verb|\citep[see][]{jon90}| & (see Jones et al., 1990) \\
\verb|\citep[see][chap.~2]{jon90}| & (see Jones et al., 1990, chap.~2) \\
\verb|\citet*{jon90}| & Jones, Baker, and Williams (1990) \\
\verb|\citep*{jon90}| & (Jones, Baker, and Williams, 1990) \\
\verb|\citet{jon90,jam91}| & Jones et al. (1990); James et al. (1991) \\
\verb|\citep{jon90,jam91}| & (Jones et al., 1990; James et al. 1991) \\
\verb|\citep{jon90,jon91}| & (Jones et al., 1990, 1991) \\
\verb|\citep{jon90a,jon90b}| & (Jones et al., 1990a,b) \\
\end{tabular}

Alternatively, use {\tt\string\citealt} and {\tt\string\citealp} to produce
a cite without parentheses:

\begin{tabular}{ll}
\textbf{Command} & \textbf{Output} \\
\verb|\citealt{jon90}| & Jones et al. 1990 \\
\verb|\citealt*\{jon90}| & Jones et al., 1990 \\
\verb|\citealp*\{jon90}| & Jones, Baker, and Williams, 1990 \\
\verb|\citealp{jon90,jam91}| & Jones et al., 1990; James et al., 1991 \\
\verb|\citealp[pg.~32]{jon90}| & Jones et al., 1990, pg.~32 \\
\end{tabular}

\clearpage

Finally, the {\tt\string\citeauthor} and {\tt\string\citeyear} commands can
be used to print only the author or year portion of the citation:

\begin{tabular}{ll}
\textbf{Command} & \textbf{Output} \\
\verb|\citeauthor{jon90}| & Jones et al. \\
\verb|\citeauthor*{jon90}| & Jones, Baker, and Williams \\
\verb|\citeyear{jon90}| & 1990 \\
\verb|\citeyearpar{jon90}| & (1990) \\
\end{tabular}

\end{document}

